Pixel-level Scene Understanding in One Token: Visual States Need What-is-Where Composition

For robotic agents operating in dynamic environments, learning visual state representations from streaming video observations is essential for sequential decision making. Recent self-supervised learning methods have shown strong transferability across vision tasks, but they do not explicitly address what a good visual state should encode. We argue that effective visual states must capture what-is-where by jointly encoding the semantic identities of scene elements and their spatial locations, enabling reliable detection of subtle dynamics across observations. To this end, we propose CroBo, a visual state representation learning framework based on a global-to-local reconstruction objective. Given a reference observation compressed into a compact bottleneck token, CroBo learns to reconstruct heavily masked patches in a local target crop from sparse visible cues, using the global bottleneck token as context. This learning objective encourages the bottleneck token to encode a fine-grained representation of scene-wide semantic entities, including their identities, spatial locations, and configurations. As a result, the learned visual states reveal how scene elements move and interact over time, supporting sequential decision making. We evaluate CroBo on diverse vision-based robot policy learning benchmarks, where it achieves state-of-the-art performance. Reconstruction analyses and perceptual straightness experiments further show that the learned representations preserve pixel-level scene composition and encode what-moves-where across observations. Project page available at: https://seokminlee-chris.github.io/CroBo-ProjectPage.

==> tables/design_choices.tex <==

\iffalse
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{lccccc}
\toprule
 & knob & light & sdoor & ldoor & micro \\
\midrule
TP   & 44.4{\tiny$\pm$3.7} & 67.6{\tiny$\pm$6.9} & 96.4{\tiny$\pm$1.8} & 36.8{\tiny$\pm$8.7} & 49.6{\tiny$\pm$7.6} \\
TP-C & 38.2{\tiny$\pm$3.6} & 62.8{\tiny$\pm$6.0} & 90.8{\tiny$\pm$3.7} & 22.2{\tiny$\pm$2.8} & 28.4{\tiny$\pm$2.4} \\
CroBo & \textbf{57.6}{\tiny$\pm$\textbf{8.1}} & \textbf{81.6}{\tiny$\pm$\textbf{2.1}} & \textbf{98.6}{\tiny$\pm$\textbf{1.4}} & \textbf{36.8}{\tiny$\pm$\textbf{3.8}} & \textbf{50.4}{\tiny$\pm$\textbf{5.8}} \\
\bottomrule
\end{tabular}
\caption{Branch ablation. TP reconstructs patches at $t{+}k$ from $\text{CLS}_t$ and visible patches at $t{+}k$. TP-C performs the same on cropped images. CroBo combines both. Success rate (\%)$\pm$std on Franka Kitchen.}
\label{tab:branch_ablation}
\end{table}
\fi 
%병주) 사실 RSP는 메인테이블에서 조차 +- 자체를 표기 안했는데, ablation에서 표기 안해도 될거 같음
%병주) table은 caption이 위로 가는게 CVPR 포맷임
%병주) 약어쓸때 첫 글자 대문자가 낫지 않을까 생각
%병주) TP, TP-C, CroBo는 우선 약자만 보고 무슨말인지 알 수 없을 뿐만 아니라 통일성도 없음. 할거면 TP, TP-C, C 이래야 할거 같은데. CroBo가 아니라
%병주) source와 target view 사이의 관계에 대한 ablation study임.
%병주) 순서상 ours가 중간인게 좋을듯?
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.07}
\caption{
Ablation on the construction of the target view.
Models are pre-trained on Kinetics-400 for 100 epochs and evaluated on Franka Kitchen (success rate \%).
``Time'' uses a future frame at time $t+k$ as the target view.
``Crop'' uses a cropped local region as the target view.
Our method is highlighted in \colorbox{gray!15}{gray}.
}

\begin{tabular}{cc|ccccc}
\toprule
Time & Crop 
& Knob1 & Light & Sdoor & Ldoor & Micro \\
\midrule

\ding{51} & {}
& 44.4 & 67.6 & 96.4 & \textbf{36.8} & 49.6 \\

\rowcolor{gray!15} {} & \ding{51}
& \textbf{57.6} & \textbf{81.6} & \textbf{98.6} & \textbf{36.8} & \textbf{50.4} \\

\ding{51} & \ding{51}
& 38.2 & 62.8 & 90.8 & 22.2 & 28.4 \\


\bottomrule
\end{tabular}
\label{tab:branch_ablation}
\end{table}
